An Investigation of Robustness of LLMs in Mathematical Reasoning: Benchmarking with Mathematically-Equivalent Transformation of Advanced Mathematical Problems

Frontier large language models (LLMs) now reach near-ceiling accuracy on standard mathematical-reasoning benchmarks and gold-medal-level performance at the International Mathematical Olympiad. As these benchmarks saturate and their items leak into training data, a high score no longer shows whether a model reasons robustly or which component of its reasoning fails. To evaluate reasoning while keeping results informative and failures diagnosable, we propose GAP (Generalisation-and-Perturbation), a methodology that automatically generates mathematically equivalent variants of existing mathematics problems at scale using two disjoint, interpretable transformations: (1) surface renames, probing the binding between identifiers and latent variable roles, and (2) kernel rewrites, probing whether a high-level proof plan survives a change of mathematical setting. Compared with existing benchmarks, GAP has two key benefits: (1) novel, likely unseen variants mitigate data leakage, and (2) performance across transformation families enables failure diagnosis, each transformation testing a hypothesis about the cause of failure. We instantiate GAP on all 1,051 William Lowell Putnam Competition problems from 1938 to 2024, adding 5,255 unseen variants to form PutnamGAP, a 6,306-item competition-level mathematics corpus and the first public machine-readable dataset from the full Putnam archive. Using PutnamGAP, we evaluated 18 commercial and open-source models spanning sizes and providers. Accuracy drops across all models and variant families, most severely under kernel rewrites. This gap does not close with model strength, suggesting that even the strongest models' dominant weakness is transferring a proof plan to a changed mathematical setting, rather than handling surface changes. Further analysis provides finer failure diagnoses and potentially useful insights for improving LLM reasoning.

==> checklist_neurips.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The introduction states four contributions (framework, benchmark, evaluation, mechanism analysis) that are developed in Sections~3--5 and validated empirically.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: Section~6 (Discussion) includes a dedicated Limitations subsection covering single-pass evaluation, single judge family, English-only scope, and competition-style restriction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{}
    \item[] Justification: The soundness bound $\delta \leq 14\,\varepsilon^{KJ}$ is stated with its independence assumption in Section~3.2 and derived in full in Appendix~\ref{app:delta_soundness}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: All prompts are in Appendix~\ref{app:prompts}, pipeline configuration and pseudocode in Appendices~\ref{app:pipelines} and~\ref{app:algorithm}, grading rubrics and model identifiers are fully specified.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The full PutnamGAP dataset, generation pipeline code, raw model outputs, and evaluation scripts are publicly released alongside this submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: No training is performed. Evaluation uses a unified zero-shot prompt (Appendix~\ref{app:prompts}), and all 18 model identifiers, temperature settings, and grading criteria are specified in Sections~4 and~5.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Paired two-proportion $z$-tests, McNemar tests, sign tests, Cohen's $d$ with bootstrap CIs, and Wilson CIs are reported throughout Sections~4--5 and Appendix~\ref{app:supplementary}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: Wall-clock times for the surface and kernel pipelines are given in Section~3.2. API-based inference costs and compute details are in Appendix~\ref{app:compute}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: The work is an evaluation benchmark for mathematical reasoning; it involves no human subjects, personal data, or dual-use concerns.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: The contribution is an evaluation methodology and benchmark for mathematical reasoning. It does not introduce new model capabilities and poses no foreseeable negative societal impact.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: The released asset is a dataset of mathematical competition problems and their equivalence-preserving variants; it poses no misuse risk.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: The Putnam source materials are credited to the four MAA Press monographs (cited in Section~4.1); fair-use terms and the MAA licence are discussed in Appendix~\ref{app:sources}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{}
    \item[] Justification: PutnamGAP is documented in Section~4 (scale, coverage, quality control) with a concrete JSON example in Appendix~\ref{app:dataset_example}. The dataset and code are included with the submission.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
    \item[] Answer: \answerNA{}
    \item[] Justification: No crowdsourcing or human-subjects research was conducted.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: No human subjects were involved in this research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    \item[] Answer: \answerYes{}
    \item[] Justification: LLMs are central to the pipeline: o3 is used for surface-variant generation, kernel-variant generation, multi-judge verification, and grading. All roles are described in Sections~3.2--3.3 and Appendix~\ref{app:robustness}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sections/06_implications.tex <==
% =====================================================================
% 06 - Implications
% =====================================================================

The structural dichotomy identifies two failure regimes but does not pinpoint their internal substrates. Combining GAP's perturbation-axis decomposition with model-internal probing --- activation patching \citep{meng:2022}, logit lens \citep{belrose:2023}, or steering-vector analysis \citep{turner:2023} on open-weight models --- could localise each regime to specific layers or attention heads, bridging the gap between our black-box signatures and a mechanistic account.\looseness=-1

On the intervention side, the rescue asymmetry suggests that inference-time interventions are regime-specific. Canonical-prefix scaffolding recovers a significant fraction of surface failures but leaves kernel failures largely intact. Designing kernel-side interventions --- whether through parameter-aware prompting, retrieval of structurally analogous solved instances, or fine-grained plan decomposition --- is an open problem that the two-regime framing now makes precise.\looseness=-1

Beyond the Putnam setting, the behavioural transfer to MATH \citep{hendrycks:2021} and ALG514 \citep{kushman-etal-2014-learning} confirms that the pipeline generalises, but the trajectory-level dichotomy has so far been established only on PutnamGAP. Reproducing the \S\ref{sec:dissociation} dissociation on other corpora --- with full trajectory capture and structural-overlap analysis --- would test whether the two-regime structure is a general property of LLM mathematical reasoning or a consequence of competition-level difficulty.

We close with a practical recommendation. Evaluations that report only aggregate accuracy or a single robustness index over mixed transformation types conflate the two regimes. At minimum, surface and kernel drops should be reported separately; where feasible, paired structural overlap and prefix-restoration rebound rates should accompany accuracy, so that readers can distinguish representation-level fragility from plan-level fragility without re-running the models.


==> sections/07_robustness.tex <==
% =====================================================================
% 07 - Reliability of the GAP Pipeline
% =====================================================================

\subsection{Robustness of surface variations}

Surface variations are produced by deterministic string substitution from the dataset's rename map. A post-validator rejects any collision with existing identifiers. Because the operation is a pure rename --- no equation, constant, or solution step is altered --- mathematical equivalence holds by construction. No judge, no grading model, and no theorem-proving capability is involved. The structural-overlap analysis in \S\ref{sec:dissociation}, which is the paper's headline mechanistic finding, is computed entirely from these deterministic rename maps and the models' own trajectories, with zero LLM annotation at any stage.

\subsection{Robustness of kernel variations}

Every LLM call in the kernel pipeline operates in an information-asymmetric verification role: the judge sees the original problem, the reference solution, the regenerated proof, and the candidate variant, and is asked whether equivalence holds step by step. This is strictly easier than solving the problem from scratch --- the judge need not search the solution space, only check a presented chain. Under an empirical single-judge error rate $\varepsilon \leq 0.04$, the two-in-a-row unanimous rule across $J{=}5$ judges and $T{=}15$ repair iterations yields a soundness bound $\delta \leq 14\,\varepsilon^{KJ} < 10^{-10}$ on a flawed variant surviving the loop. The bound holds at $\varepsilon = 0.08$ with $\delta < 10^{-8}$. A $10\,\%$ manual audit on accepted variants found no substantive errors.

\subsection{Robustness of grading}

Three independent providers (GPT-4o, Claude-Sonnet-4, Gemini-2.5-flash) grade the same 50 stratified solutions; pairwise Cohen's $\kappa$ ranges from $0.96$ to $1.00$, with agreement on 49--50 of 50 cases. On calculation problems, a strict string-match grader runs in parallel with the LLM grader; disagreement is below $1\,\%$. A separate $10\,\%$ random-sample human audit on the full grading run confirms precision and recall above $97\,\%$.

\subsection{Robustness across datasets}

We apply the same surface pipeline to 159 MATH Level 4--5 problems \citep{hendrycks:2021} (six models) and to ALG514 \citep{kushman-etal-2014-learning} (one model) to verify that the behavioral asymmetry is not specific to Putnam. All 12 (model, surface-variant) cells on MATH show negative paired drops; 8 of 12 are individually significant by McNemar at $p < 0.05$, with the largest being gpt-4.1-nano on GS ($-21.4$~pp, $p = 1.2 \times 10^{-6}$). On ALG514, accuracy falls from $93.6\%$ to $90.9\%$ under DLC ($p = 0.024$) and to $89.3\%$ under GS ($p = 0.002$). We claim behavioral transfer of the framework, not mechanism-level reproduction: trajectory-level dissociation on these corpora requires trajectory-capturing reruns and is left to future work.

\subsection{The verification gap as a design principle}

GAP is designed around a structural asymmetry between the solver and the verifier. The models under evaluation must solve a problem from scratch with no reference answer; every LLM inside the pipeline --- generators, judges, graders --- operates with the reference answer, the canonical solution, or both already in hand. Checking a presented proof against a known answer is strictly easier than producing one, so the pipeline does not require frontier-level reasoning from any of its components. This verification gap is what makes multi-judge consensus, bounded repair loops, and cross-provider agreement effective: each mechanism amplifies a base reliability that is already high because the task is verification, not generation.


==> sections/08_conclusion.tex <==
% =====================================================================
% 08 - Conclusion
% =====================================================================

Accuracy on a fixed benchmark cannot tell whether a model is reasoning
robustly or matching surface cues. We presented \textbf{GAP}, an
evaluation framework whose equivalence-preserving transformations
split into two disjoint, mechanism-aligned families: \emph{surface
renames} probing the binding between identifiers and latent variable
roles, and \emph{kernel rewrites} probing whether a high-level proof
plan survives a change of mathematical setting. Instantiated on every
William Lowell Putnam problem from 1938 to 2024, GAP yields
\textsc{PutnamGAP}: 1{,}051 canonical items paired with 5{,}255
aligned variants, the kernel pipeline carrying an architectural
soundness bound of $\delta < 10^{-10}$. Because that pipeline can
resample arbitrarily many fresh items after a model is trained,
benchmark contamination becomes a generative-pipeline problem rather
than a one-shot data problem.

Across 18 commercial and open-source models, accuracy drops on every
transformed family, the largest losses come from kernel rewrites, and
the kernel--surface gap \emph{widens} with model strength. The
decomposition further exposes a mechanism-level dichotomy that is
invisible from aggregate accuracy: surface failures drift from the
model's own original-correct trajectory and largely recover when an
item-specific framing is restored, while kernel failures drift from
the canonical proof plan itself and resist the same intervention.
Robustness in advanced mathematical reasoning is therefore not a
scalar to optimise but at least two distinct properties to audit, and
the regime-specific recommendations of \S\ref{sec:implications}
follow directly.

\paragraph{Limitations and future work.}
We evaluate models under a single zero-shot pass (no test-time
scaling); the $J{=}5$ kernel judges are drawn from a single model
family; the structural diagnostic requires visible reasoning chains;
and \textsc{PutnamGAP} is English-only and competition-style. Natural
extensions are heterogeneous verifier ensembles that pair LLMs with
symbolic checkers (Lean, SMT), porting the two-pipeline construction
to adjacent STEM corpora with different proof structures, and
applying surface and kernel transformations during fine-tuning to
test whether the relevant invariances are learnable rather than
incidental.

GAP reframes the question. Progress in mathematical
reasoning is measured not by accuracy on a fixed benchmark, but by
which components of reasoning -- representation \emph{and} plan --
survive equivalence-preserving change.

